Search for Stellar Flybys in the Sco-Cen OB Association with the Gaia DR2

High-contrast imaging studies of debris disks have revealed a significant diversity in their morphologies, including large-scale asymmetries. Theories involving stellar flybys, an external source of gravitational disturbance, have offered a plausible explanation for the origin of these morphological variations. Our study is an experiment to gain empirical evidence that has been lacking from such theories. We explore this paradigm by using astrometric and radial velocity measurements from the Gaia DR2 and ground-based observations to trace the trajectories of 625 stars in the Sco-Cen OB Association from 5 Myr in the past to 2 Myr in the future. We identified 119 stars that had at least one past flyby event occurring within one Hill radius, and 23 of these experienced flybys within 0.5 Hill radius. We found no evidence of a significant correlation between the presence of flyby events and infrared excess detections, although the sample is not uniformly sensitive to infrared excess emission. Ten stars that had past flyby events host resolved circumstellar disks that appear relatively symmetric in the existing data except for the circumbinary disk surrounding HD 106906. We determined the trajectory and relative velocity of each of these flyby events, and compared these to the geometry of the spatially-resolved disks. Future work is needed to measure the kinematics of lower mass stars and to improve sensitivity to circumstellar disks for the entire sample.

==> old-text.tex <==
\subsubsection{V856 Sco (HD 144668)}\label{dis:v856sco}
\edit1{This Herbig Ae star is the only one in this section which we have identified close ($d_\mathrm{ca}<1\,\mathrm{pc}$) field star flybys. It encounters THA 15-34 (M6) at $d_\mathrm{ca}=0.61_{-0.35}^{+61}\,\mathrm{pc}$ and $t_\mathrm{ca} = -0.25_{-0.37}^{+0.33}\,\mathrm{Myr}$. It also encounters SZ 106 (M2.5) at $d_\mathrm{ca}=0.31_{-0.22}^{+0.40}$ pc and $t_\mathrm{ca} = -0.05_{-0.24}^{+0.24}$ Myr -- accounting for the uncertainties, they are currently undergoing the approach. Compact circumstellar material around V856 Sco with $R\sim3$ au was detected at 8-13 $\mu$m emission by \cite{2006A&A...458..235P} using long-baseline interferometry with VLTI. The mid-IR emission was again detected by \cite{2011ApJ...737...57M} at 12  $\mu$m and 18 $\mu$m, but the disk is not resolved. \cite{2017A&A...599A..85L} observed the star with \textit{H}-band PIONIER/VLTI interferometer and constrained the disk orientation; the image reconstruction of this data by \cite{2020A&A...636A.116K} shows consistent results, which we used to carry out the calculation of flyby angle. The small disk ($\sim10$ au) around V856 Sco is likely due to the presence of a companion \citep{1995A&A...296..463S, 2017A&A...603A..21G}, and we consider the dynamical effects of the flybys to be minor. } 


V856 Sco & THA 15-34 & $2.45_{-1.66}^{+2.44}$ & $0.61_{-0.35}^{+0.61}$ & $-0.25_{-0.37}^{+0.33}$ & $41.38_{-2.87}^{+4.16}$ & $7.93_{-2.39}^{+2.42}$ & 6\\
{} & SZ 106 & $1.65_{-1.15}^{+1.78}$ & $0.31_{-0.22}^{+0.40}$ & $-0.05_{-0.24}^{+0.24}$ & $41.90_{-2.40}^{+3.30}$ & $9.87_{-2.57}^{+2.59}$ & \\\hline



\edit1{Nonetheless, the possibility of very close ScoCen--Field encounters are not ruled out. Due to the overwhelming number of field star flybys, we focused on those with  $d_\mathrm{ca}\lesssim1\,\mathrm{pc}$ and $v_\mathrm{rel} \lesssim 10\,\mathrm{km/s}$, i.e. the most dynamically interesting ones. We identified 10 field star flybys, and only one has a resolved circumstellar disk V856~Sco, discussed in Section~\ref{dis:v856sco}. However, it is worth pointing out that a non-negligible fraction of flyby stars within the field star sample may be unidentified Sco-Cen members due to uncertainties on their kinematics. For example, both TWA 30 A and B are among the 10 field star flybys, but only A is included the Sco-Cen sample, whereas B---a bound companion of A---belongs to the field sample.}
